Integrating Artificial Intelligence into Weapon Systems

The integration of Artificial Intelligence (AI) into weapon systems is one of the most consequential tactical and strategic decisions in the history of warfare. Current AI development is a remarkable combination of accelerating capability, hidden decision mechanisms, and decreasing costs. Implementation of these systems is in its infancy and exists on a spectrum from resilient and flexible to simplistic and brittle. Resilient systems should be able to effectively handle the complexities of a high-dimensional battlespace. Simplistic AI implementations could be manipulated by an adversarial AI that identifies and exploits their weaknesses. In this paper, we present a framework for understanding the development of dynamic AI/ML systems that interactively and continuously adapt to their user's needs. We explore the implications of increasingly capable AI in the kill chain and how this will lead inevitably to a fully automated, always on system, barring regulation by treaty. We examine the potential of total integration of cyber and physical security and how this likelihood must inform the development of AI-enabled systems with respect to the "fog of war", human morals, and ethics.

==> src/conclusion.tex <==
%Finished 4.26.19 3:30 pm Phil
\section{Conclusion}
In this paper, we have presented a framework or rough roadmap for approaching the problem of integrating AI and ML into weapons systems and the killchain. We believe that a transdisciplinary approach is required for an effort such as this, given that the potential outcomes can be fraught with unexpected and dangerous consequences. This is more than simply taking existing AI approaches and layering them on top of existing weapons systems. \enquote{Innovations like artificial intelligence, ubiquitous sensors, big data, and virtual reality raise significant questions about safety, security, privacy, and liability, and commercial markets for these technologies cannot thrive without a clear roadmap of how we will approach governing their development and use.} \cite{carter2018chinese}

This roadmap only begins with an examination of how humans become overloaded in combat situations and how machines can seamlessly take up that load, allowing the human operator to function meaningfully in the battlespace. We should proceed with a deep awareness that the steps we take may be on a path to human obsolescence as combatants. The decision to proceed on this path should be well informed and involve all members of our societies. The research that we do now informs the development of these systems. This can inform policy makers more deeply about the risks and rewards of proceeding. Particularly given that other players are deeply engaged in the weaponization of AI, we would be foolish not to research and experiment with the development of highly capable systems. But we believe that a better answer may be to create an understanding in the citizenry that, like chemical and biological weapons, for weaponized AI, \enquote{The only winning move is not to play}, and to support regulation and prohibition.

==> src/cover.tex <==
% COVER PAGE (not to exceed one page):
% The whitepaper cover page shall include at a minimum: Title of the whitepaper, name of the individual and organization submitting the whitepaper, the research area and number against which the whitepaper is submitted, and the TPOC name. 

%Title, Period of Performance, Estimated Cost, Name/Address of Company, Technical and Contracting Points of Contact (phone and email)

\title{\textbf{Integrating Artificial Intelligence into the Killchain} \\
	FOCUS AREA 3 - Machine Intelligence \\
	Period of performance: June - Dec 2019  (or 6 months duration depending on award date) \\
	Estimated cost: \$475,000 \\
	ASRC Mission Solutions - Alaska Native Corp. 8(a) Minority-owned \\
	CAGE: \hl{ADD CAGE CODE HERE},   EFT: \hl{ADD EFT CODE HERE} \\
	Solicitation BAA FA8750-18-S-7014\\
	U.S. Air Force BAA Whitepaper\\
	\begin{figure} [h]
		\centering
		\includegraphics[width = 15em]{asrc-federal-mission-solutions-logo-fullcolor-white-bkg.jpg}
	\end{figure}
	}
\author{Philip Feldman\\
	410.300.7293\\
	philip.feldman@asrcfederal.com
	\and
	TPOC: Aaron Dant \\
	301.661.3361\\
	aaron.dant@asrcfederal.com
}


\pagenumbering{gobble} 

==> src/currentWork.tex <==
\section{Current Military Use of AI}%
\label{sec:current_work}

Although some peripheral military applications exist, the vast majority of
modern AI is biased towards the commercial sector~\cite{chui2018notes}.  In
general, machine learning products take over areas of cognition that humans
would otherwise have to do, including classifying images, translating
text, or driving cars.  In all these cases, the operating assumption and
experience adheres to the idea that "bigger is better".  For example, Google's
BERT model~\cite{DevlinBERT2018}, when trained using one billion parameters,
can produce a prediction of the Wikipedia entry for Abraham Lincoln that is
startlingly good.  At 10 million parameters, BERT is not much better than
syntactically correct random words~\cite{tensorflow_2019}.  However, the very
size and sophistication of these models create an implicit risk for combat
systems.

Such giant models take considerable time and effort to produce, and they only
provide value if they can be deployed and used at scale.  The effort involved
in making such a large model has meant that methods have been used to adapt
the latent information encoded into the model to other domains.  A model
trained to recognize general classes of objects (a can, for example) can be
retrained to recognize specific instances (Coke vs.  Campbell) This has led to
the the subfield of \enquote{transfer learning}, where a pre-trained model is
adapted by adjusting the weights in the last \textit{n} layers such that a
model trained on Wikipedia text can be used to create news articles
instead~\cite{pan2010survey}.

For combat systems, these models create an inherent risk.  Since academic and
corporate models are few and often in the public domain, a malicious actor can
simply download and study them for areas where they can be manipulated to
respond incorrectly to a particular set of
stimuli~\cite{goodfellow2014explaining}.  Since transfer learning changes only
a small part of the network, these vulnerabilities would likely exist
regardless of how the model has been adapted.  This places any combat system
based on one of these models at risk for undetectable exploitation.  Models
developed in secure environments based on real and simulated data may be
significantly more secure from exploitation, but with a correspondingly higher
cost to develop.

Another area of research is the development of \enquote{edge neural networks}.
This technology, emerging from the ongoing development of the Internet of
Things (IoT), places custom hardware that supports inference and transfer
learning on large models on a device-by-device basis.  This type of approach
could allow a model that is created using generic combat capabilities to
\enquote{learn} as it is used in a unique environment or situation using a
process that Google calls \textit{imprinting}
\footnote{coral.withgoogle.com/tutorials/edgetpu-api/}.  These modified
networks can then update the master model with lessons learned in the field
through a process called \enquote{Federation}
\footnote{www.tensorflow.org/federated}.  This could provide much-needed
adaptability, though it leaves open questions about verification and testing
of these field-developed models.


==> src/taskObjective.tex <==
\section{Task Objective}
Even without exacerbating conditions such as combat, humans often find making the right decision under stress (particularly with incomplete information)  difficult, and the tendency to depend on authorities, either human or machine, can lead to disastrous outcomes\cite{ferraris2003nasa, clark2011gps}. 

Machine learning and artificial intelligence hold the promise of being able to integrate dynamically into the human decision making process in a way that previous technologies could not, and to make this integration responsive to the operator's cognitive load. 

But once AI decision-making is implemented, it should be assumed that an adversarial AI-enhanced actor is doing the same. As much as AI may advantage the warfighter, it also presents an opportunity to the adversary to induce its opponent's AI to misbehave in ways that humans may not be able to detect until too late\cite{staff2014joint}. 

\subsection{Background}
Although the battlespace has been getting progressively faster and more complicated as tactics change, technologies emerge and communication improves, the fundamental processes have been unchanged for centuries - opposing commanders observe the evolving battlespace, attempt to understand and model the space so that the actions they direct lead to positive outcomes. Of course, what makes this difficult is that the adversary is doing the same thing, leading to a co-evolving physical and information environment that is difficult to predict with any certainty. 

These rapidly co-evolving battlespace dynamics are one of the largest obstacles in involving current state-of-the-art machine learning systems. Currently, the best AI is based on enormous networks that are trained for days against massive datasets. The timeframes involved in this process do not afford the rapid updates that human interaction requires. Recent advances in techniques such as meta-learning allow for some flexibility in updating a large model, though it is unclear as to the range, scope and flexibility of these approaches with respect to combat conditions.

To address both the promise and the risks of adding lethal combat capabilities to AI systems, we need to establish a development framework that emphasizes human control over the behaviors of such systems, regardless of how sophisticated they become. At the core, we believe that these aspects of human control must include the following:

\begin{itemize}
	\item \textit{Interactivity}: Users need to be able to explore and adjust the behavior of the system in such a ways as to be able to perceive the change that they have made and validate that they system exhibits a more \enquote{correct} behavior than before the intervention
	\item \textit{Transparency}: Although we believe that intelligent machines may never truly be able to explain \textit{why} they did something, they should be able to point to the sources that they used to learn this behavior, be it a document or hands-on instruction by an expert user.
	\item \textit{Resilience}: A system cannot be brittle. It needs to be able to handle gracefully and recover from situations intended to place it into an overloaded condition. It should be able to indicate that it is operating with low confidence, but it cannot simply \textit{freeze}.
\end{itemize}

Even though the goal of adding AI to the battlespace is to augment humans, there are ramifications to that goal that extend beyond that very constrained use case and need to be considered earlier rather than later. The issue is that intelligent augmentation in combat means that even at the beginning, the results of this effort will be (constrained) artificially intelligent fighting machines. If AI systems are effective as aids, there will always be pressure to increase the level of assistance to the warfighter, gradually pushing the human out of the loop to a supervisory role, and then finally to the role of a "killswitch operator" monitoring always-on, Lethal Autonomous Weapons Systems (LAWS).

\subsection{The role of humans}
Because of the rate of technological development in the AI/ML space, we believe that the role of humans in combat systems, \textit{barring regulation through treaty}, will become more peripheral over time. As such, it is critical to ensure that our design decisions and the implementations of these designs include at the core the values that we wish to express as a national and global culture.

\subsubsection{Human-in-the-loop}
The starting point for many intelligent systems begins with the tight integration of human and machine in the weapon system. For example, firing solutions automatically include superelevation and lead. Missiles announce when they have a lock. These affordances increase the capability of the warfighter and leave little ambiguity as to what the weapons system will do once the trigger is pulled. If fault has to be found, it will be the human that must bear the responsibility.

But in more ambiguous circumstance, such as friend-or-foe identification (IFF), the data used to make the calculation will be in the possession of the system, not the user. Imagine, for example, a case where an IFF transponders have been known to be spoofed by the adversary, and a large, slow moving aircraft identifying as civilian has been detected entering the battlespace on what seems to be a hostile approach, and only a short time to make a decision.  

From a user perspective, there are three presentations. 
\begin{enumerate}
	\item The system can declare that it has identified the aircraft as hostile and provide a lock. 
	\item The system can declare the aircraft as friendly and open a channel to warn
	\item The system can present a set of ranked recommendations and provide a set of options to the user
\end{enumerate}

Of these, it would seem like the third option is the best utilization of the human-in-the-loop philosophy. However, it discounts the human tendency to trust the system if it's behaved correctly in the past. The user may spend some time evaluating the list of options the first few times, but if the system places the correct option at the top of the list often enough, the human user will begin to feel comfortable with simply selecting the first option. Increase the time pressure, and the human will simply become a rubber stamp, as the penalty for slow response may be worse than the wrong response.

A way to address this issue is to change the way that the system is trained and presents its recommendations. If the system is trained by a set of known individuals, and the provenance of the decision of the system traces back to its \enquote{mentor}, then a human user can select among a set of human recommendations. Some mentors may be training the model in the context of the current deployment and be known to the user. The human mentor embodies the trust relationship and the responsibility of the decision. This immediate, low-level and intimate relationship to the current situation is inherently more relatable to a human user and potentially more qualitatively informative than a simple ranking based on probability. 

We believe that this sort of intimate and individual training may be possible using recent advances in transfer and meta-learning\cite{yangmeta2018} may be the best answer for human-in-the-loop configurations. The machine, as it expresses the training from the human mentor can express latent information that incorporates rules of engagement that are related to the particular deployment. This approach, where the machine learning happens as close to the front lines as possible is most likely to embody appropriate responses to localized complex situations. Further, weights that are accumulated from these interactions can be brought back and integrated in the initial models, allowing them to evolve with respect to the current realities of a given battlespace.

\subsubsection{Human-on-the-loop}
As our adversaries develop their own means to overwhelm our warfighter's human cognitive capability and we work to undermine theirs, this option appears inevitable. Work is already being done in this space commercially, but for other reasons. Examples of what is essentially human-on-the-loop architectures are regularly explored now in StarCraft competitions\cite{andersen2018deep}. 

From a machine learning perspective, the difference between a StarCraft 2 environment and an Aegis battlegroup is one of scale and consequences - the technology involved would be roughly the same. Though the level of interaction in real-time is lower, there may be a way to integrate the mentor architecture described above in these systems as well. This would depend on the creation of offline wargames and simulations that can be played at rates slow enough to allow human cognition using trained experts to contribute in a meaningful way.

By running larger number of potential scenarios offline, the odds can be increased that the trained system reflects the realities of the battlespace in the particular context and environment. Additionally, separate classifier systems may be able to catalog adversary behaviors that are near the boundaries of the current trained responses. These boundaries could be detected by looking at the behavior of the systems themselves, and recognizing when they are making decisions among multiple options with divergent potential outcomes.  

\subsubsection{Human-initiated}
An extension of the human-on-the-loop approach is the human-initiated \enquote{fire and forget} approach to battlefield AI. Once the velocity and dimensionality of the battlespace increase beyond human comprehension, the level of human interactivity will be to choose the \enquote{flavor} of behavior that may be desired in a context that contains the potential for high velocity AI conflict. There will be no time to engage the system at the onset of hostilities. Rather, these systems will need to be configured and activated will before the onset of any hostility. Activating one of these systems in a conflict arena could be an extremely consequential action, as once activated, the very act of bringing it down for any reason may expose a weakness that would be exploited by an adversarial AI. It is extremely unlikely that we will be able to predict with confidence how a conflict between two equally matched, highly capable AI systems would unfold once started. These types of conflicts would have to be extensively wargamed and simulated against a wide variety of adversaries to have any level of confidence that they would behave in a way that aligns with our national values.

\subsubsection{Post-hoc forensics}
Given a battlespace so overwhelming that humans can't even be relied on to engage the system, then the human role will be that of post-hoc analysis, once hostilities have ceased, or treaties have been signed and implemented. To support this, we will need to design our systems so that the maximal amount of provenance for a decision is associated with sufficiently high-fidelity recordings of the inputs to the system so that any error or inexplicable behavior can be deciphered. Recently, some work that applies a potential approach to these sort of forensics is the concept of an \enquote{activation atlas}\cite{carter2019activation} that can show areas of conceptual conflict within a model. These sorts of approaches are nascent, but need to be vigorously explored and developed.


==> src/techSummary.tex <==
\section{Technical Summary and Proposed Deliverables}
%TODO: add a proposed deliverable to each section
An overarching bias in current AI/ML research and development is that \enquote{bigger is better}. Models have grown rapidly to the point that the largest have billions of parameters, exabytes of data, and need supercomputers to train in reasonable timeframes. This is an effective commercial and academic strategy because these models can be reused and modified using techniques such as transfer learning.

As stated earlier in the paper, we believe that military adaptation of these models contains inherent risks from a variety of human-centered perspectives. However, these areas of risk also include potential opportunities for areas of development that are unique and distinct from the focus of commercial and academic communities:

\subsection{Legal and ethical constraints} \label{sec:legal_and_ethical}
Modern AI/ML systems reflect the data that is used to train them. In commercial and academic systems, data often reflects unconscious biases that emerge in the trained behavior of the system. This type of behavior only becomes more dangerous when it is connected with the killchain. We need to develop techniques that allow us to train models that have the appropriate rules of engagement \enquote{baked in} so that they can be appropriately expressed given a particular context, ranging from wargames in peacetime to escorting an adversarial emissary to a peace conference in wartime. 

Mechanisms for these sort of legal and ethical considerations are not an area of current research, and the particular aspects of how they are expressed at various levels of abstraction is a particularly complicated problem. We have some indication that hierarchies of ML and human ensembles might be able to express appropriate behavior across a wide range of conditions, and that these and other approaches need to be explored deeply before we simply \enquote{bolt on} a machine learning solution to a weapons system. 

\subsubsection{Proposed Deliverable}
Create, demonstrate, and document a proof-of-concept example AI system that can be trained in an interactive way classify ethical dilemmas and rules of engagement in a simulated environment, possibly based on the work by Honovar and Ghasem-Aghaee's on neural-network-based artificial moral agents\cite{honarvar2009artificial}. This framework provides a generalized evaluation framework for evaluating computational responses to ethical issues. 

\subsection{Mapping and traceability}
It is our strong belief that our intelligent weapons systems of the future will move and think at machine speed - many times that of their human partners. These disproportionate capabilities and the level of system trust that the human operators will inevitably place in the machines that they use create the likelihood that many lethal and sub-lethal interactions will only be analyzable in hindsight. Support needs to be built into these models that supports a recording of the inputs that led to the action or recommendation, so that the network can be analyzed, retrained, and validated so that the same mistake does not happen more than once. 

\subsubsection{Proposed Deliverable}
Create, demonstrate, and document a proof-of-concept example of a \enquote{interactively trainable} deep learning system that supports the recording of salient training episodes to the system discussed in section \ref{sec:legal_and_ethical}. We expect that this effort will incorporate recent work in attention mechanisms to indicate salient training episodes\cite{mullenbach2018explainable}.

\subsection{Diverse Redundancy} Because the creation of models is complicated and time consuming, few models are created that address the same task at the same level of sophistication. There is often only one \enquote{best} model for any set of data. In a military context, this is dangerous, as it makes any system that uses the model more predictable. 

Learning to exploit regions in the latent space of the available large models should be explored in depth. There is always the chance that less well supported actors may take advantage of these models to gain high military impact for low cost and effort. Determining how to thwart, for example, a terrorist organization that weaponizes the Inception model by using it as the basis for exploding drones that head towards generic or specific faces is almost certainly a prudent move, based on the inevitability of this type of implementation.

We believe that for military systems, redundant, diverse models need to be developed and regularly revisited so that any adversary who obtains a system that expresses one model will not be able to trust that their understanding of the systems responses will be expressed in a system that they will face in battle. This need for diverse models for the same set of problems is a particular need for military systems that will not be met in the academic or commercial community, where improvements in performance are the measures of success, not survivability and ruggedness.

\subsubsection{Proposed Deliverable}
Create, demonstrate, and document a proof-of-concept example of evolutionary generation of deep neural networks such the GNARL approach, developed by as Angeline et. al.\cite{angeline1994evolutionary}. We intend to develop stochastically generated neural architectures for cases where there are known attack strategies for existing models (e.g. Su, et. al. \textit{One pixel attack for fooling deep neural networks}\cite{su2019one}). We will then evaluate these evolutionarily distinct networks for resistance to these known attacks in single and ensemble systems, exploring the concept of diverse redundancy.



